Stability Bounds for Learning-Based Adaptive Control of Discrete-Time Multi-Dimensional Stochastic Linear Systems with Input Constraints

We consider the problem of adaptive stabilization for discrete-time, multi-dimensional linear systems with bounded control input constraints and unbounded stochastic disturbances, where the parameters of the true system are unknown. To address this challenge, we propose a certainty-equivalent control scheme which combines online parameter estimation with saturated linear control. We establish the existence of a high probability stability bound on the closed-loop system, under additional assumptions on the system and noise processes. Finally, numerical examples are presented to illustrate our results.

==> leftovers.tex <==

\begin{remark} \label{remark:theorem-stability-final} 
    Theorem \ref{theorem:stability-final} provides finite-sample high probability upper bounds on the norm of the sub-sampled states $\bar{X}_{\tau}$ that holds over all sub-sampled steps $\tau \in \mathbb{N}_0$. Although the bound appears complicated, there is a clear intuition that underlies it. In particular, $\gamma$ is the failure probability associated with the unbounded stochastic disturbances due to the use of Markov's inequality, and $\delta$ is the failure probability associated with bounding the parameter estimation error over all time steps. For a fixed failure probability $\delta$, $\tau_0$ refers to the sub-sampled time step such that for all $\tau > \tau_0$, 1) $e(\kappa \tau, \delta)$ successfully upper bounds the estimation error $|| \bar{\theta}_{\tau} - \theta ||_2$, and 2) the estimation error is sufficiently small such that $|| \bar{\theta}_{\tau} - \theta_* ||_2 \leq m_q$, allowing allowing us to bound the control signal error by $|\sat_D(-g(\bar{A}_{\tau},\bar{B}_{\tau}))-\sat_D(-g(\bar{A},\bar{B}))| \leq M_q D || \bar{\theta}_{\tau} - \theta_* ||_2$. Since $e(\kappa \tau, \delta)$ is $\tilde{O}(1/\sqrt{\tau})$ as $\tau \rightarrow \infty$ (where $\tilde{O}(\cdot)$ hides constant and logarithmic factors), then $ M_q D e(\kappa \tau, \delta) = \tilde{O}(1/\sqrt{\tau})$ with failure probability $\delta$. Thus, $\tilde{O}(1/\sqrt{\tau})$ asymptotically converges to zero, such that after some step $\tau'$, supposing that Assumption \ref{assump:large-sat-level} holds, $e(\kappa \tau, \delta)$ will be sufficiently small such that $\lambda(e(\kappa \tau, \delta)) \leq \lambda' < 1$ and $\beta(e(\kappa \tau, \delta)) \leq \beta' < \infty$ will hold, where $\lambda'=\lambda(e(\kappa \tau', \delta))$ and $\beta'=\beta(e(\kappa \tau', \delta))$, as pointed out in Remark \ref{remark:lemma-stability-deterministic-param}. Thus, for $\tau > \tau'$, we have
    \begin{align}
        &\prod_{i = \tau_0}^{\tau-1}\lambda(e(\kappa i, \delta)) \\
        &\leq (\prod_{i=\tau_0}^{\tau'-1}\lambda(e(\kappa i, \delta)))(\lambda')^{\tau - \tau'}\\
    \end{align}
    which converges to $0$ as $\tau \rightarrow 0$, and
    \begin{align}
        &\sum_{i = \tau_0}^{\tau - 1} \beta(e(\kappa i, \delta)) \\
        &\times \prod_{j=i+1}^{\tau-1} \lambda(e(\kappa i, \delta)) ) )\\
        &= \sum_{i = \tau_0}^{\tau' - 1} \beta(e(\kappa i, \delta)) \\
        & \quad \times ( \prod_{j=i+1}^{\tau'-1} \lambda(e(\kappa j, \delta)) )   (\lambda')^{\tau - \tau'}\\
        & \quad + \underbrace{\beta(\epsilon)\sum_{i = \tau'}^{\tau - 1} (\lambda')^{\tau - \tau'}}_{=\sum_{i=0}^{\tau - \tau' - 1}(\lambda')^{\tau} = \frac{1-(\lambda')^{\tau - \tau'}}{1 - \lambda'}}
    \end{align}
    holds, which converges to $\frac{1}{1-\lambda'}$ as $\tau \rightarrow \infty$. By placing these observations in the context of \eqref{eqn:theorem-stability-final-after-tau_0},  Theorem \ref{theorem:stability-final} can be interpreted as a result which provides finite-sample high probability stability bounds on the norm of the sub-sampled states. \ssnote{Although this is nice result, we point out that by choosing a larger $\tau'$, a smaller $\lambda'$ can always be found, and so our observations here do not fully convergence properties of the bound in \eqref{eqn:theorem-stability-final-after-tau_0}.}
\end{remark}

\begin{corollary} \label{corollary:encoding-stability-remark}
    Suppose Assumptions \ref{assump:disturbance}, \ref{assump:reachable}, \ref{assump:exciting-noise}, \ref{assump:disturbance-bounds}, \ref{assump:large-sat-level}, and \ref{assump:bmsb} hold. Fix $\delta \in (0,1)$ and $\epsilon \in (0, || \mathcal{R}_* ||_2^{-1} M_q^{-1} (\kappa,A,B) D^{-1} \big ( \frac{D}{|| \mathcal{R}_*^{\dagger} ||_2} - \log ( M_{\bar{V}} M_{\bar{W}} ) \big ) )$. Then, for all $\tau \geq \tau'$, we have
    \begin{align}
        |\bar{X}_{\tau}| &< \log ( \frac{2}{\delta} ( e^{||A||_2^{\kappa \tau_0} | x_0 |} \\
        &\quad \times ( e^{||\mathcal{R}_* ||_2 D} M_{\bar{V}} M_{\bar{W}})^{\sum_{i=0}^{\tau_0-1} || A||_2^{\kappa i}}  \\
        & \quad \times  (\prod_{i=\tau_0}^{\tau'-1}\lambda(e(\kappa i, \delta/2)))(\lambda(\epsilon))^{\tau - \tau'} \\
        & \quad + \sum_{i = \tau_0}^{\tau' - 1} \beta(e(\kappa i, \delta/2)) \\
        & \quad \times ( \prod_{j=i+1}^{\tau'-1} \lambda(e(\kappa j, \delta/2)) )   (\lambda(\epsilon))^{\tau - \tau'}\\
        & \quad + \beta(\epsilon) \frac{1 - (\lambda(\epsilon))^{\tau - \tau'}}{1 - \lambda(\epsilon)}) )
    \end{align}
    with probability at least $1 - \delta$, where
    \begin{align}
        \tau' &= \min \{ \tau \in \mathbb{N} \mid \tau \geq \tau_0, e(\kappa i, \delta/2) \leq \epsilon \text{ for all } i \geq \tau \}.
    \end{align}
\end{corollary}

\begin{proof}
    Suppose $\tau \geq \tau'$. Then,
    \begin{align}
        &\prod_{i = \tau_0}^{\tau-1}\lambda(e(\kappa i, \delta/2)) \\
        &\leq (\prod_{i=\tau_0}^{\tau'-1}\lambda(e(\kappa i, \delta/2)))(\lambda(\epsilon))^{\tau - \tau'} \label{eqn:corollary-encoding-stability-remark-1}
    \end{align}
    holds, alongside
    \begin{align}
        &\sum_{i = \tau_0}^{\tau - 1} \beta(e(\kappa i,\delta/2)) \\
        &\times \prod_{j=i+1}^{\tau-1} \lambda(e(\kappa j,\delta/2)) ) )\\
        &= \sum_{i = \tau_0}^{\tau' - 1} \beta(e(\kappa i,\delta/2)) \\
        & \quad \times ( \prod_{j=i+1}^{\tau'-1} \lambda(e(\kappa j,\delta/2)) )   (\lambda(\epsilon))^{\tau - \tau'}\\
        & \quad + \beta(\epsilon)\sum_{i = \tau'}^{\tau - 1} (\lambda(\epsilon))^{\tau - i - 1} \\
        &= \sum_{i = \tau_0}^{\tau' - 1} \beta(e(\kappa i,\delta/2)) \\
        & \quad \times ( \prod_{j=i+1}^{\tau'-1} \lambda(e(\kappa j,\delta/2)) )   (\lambda(\epsilon))^{\tau - \tau'}\\
        & \quad + \beta(\epsilon) \frac{1 - (\lambda(\epsilon))^{\tau - \tau'}}{1 - \lambda(\epsilon)}. \label{eqn:corollary-encoding-stability-remark-2}
    \end{align}
    Then conclusion then follows by applying Theorem \ref{theorem:stability-final} with $\delta \leftarrow \delta/2$ and $\gamma \leftarrow \delta/2$, then applying the bounds in \eqref{eqn:corollary-encoding-stability-remark-1} and \eqref{eqn:corollary-encoding-stability-remark-2}.
\end{proof}

\begin{theorem} \label{theorem:simplified-bound-v2}
     Suppose Assumptions \ref{assump:disturbance}, \ref{assump:reachable}, \ref{assump:exciting-noise}, \ref{assump:disturbance-bounds}, \ref{assump:large-sat-level}, and \ref{assump:bmsb} hold. Fix $\tau \in \mathbb{N}_0$, and $\delta \in (0,1)$. The following statements hold with probability at least $1-\delta$. If $0 \leq \tau < \tau_w$, 
     \begin{align}
         | \bar{X}_{\tau} | < \log (\frac{2}{\delta}) + \log ( e^{|x_0|} ( e^{|| \mathcal{R} ||_2 D} M_{\bar{V}} M_{\bar{W}} )^{\tau} ).
     \end{align}
     If $ \tau_w \leq \tau < \tau_s$,
     \begin{align}
         | \bar{X}_{\tau} | &< \log (\frac{2}{\delta}) + \log ( \underbrace{ \frac{e^{ \frac{1}{2} ( \frac{D}{|| R^{\dagger} ||_2} + \log (M_{\bar{V}} M_{\bar{W}}) ) }}{1 - e^{-\frac{1}{2}(\frac{D}{||\mathcal{R}^{\dagger}||_2} - \log ( M_{\bar{V}} M_{\bar{W}}))}}}_{\mathcal{S}_w} +  \\
        & \quad + \underbrace{ e^{|x_0|} ( e^{|| \mathcal{R} ||_2 D} M_{\bar{V}} M_{\bar{W}} )^{\tau_w} e^{-\frac{1}{2}( \frac{D}{|| \mathcal{R}^{\dagger} ||_2} - \log(M_{\bar{V}} M_{\bar{W}}) )(\tau - \tau_w)} - e^{ \frac{1}{2} ( \frac{D}{|| R^{\dagger} ||_2} + \log (M_{\bar{V}} M_{\bar{W}}) ) } \frac{ e^{-\frac{1}{2}(\frac{D}{||\mathcal{R}^{\dagger}||_2} - \log ( M_{\bar{V}} M_{\bar{W}}))(\tau - \tau_w)}}{1 - e^{-\frac{1}{2}(\frac{D}{||\mathcal{R}^{\dagger}||_2} - \log ( M_{\bar{V}} M_{\bar{W}}))}}}_{\mathcal{T}_w} ).
     \end{align}
     If $ \tau \geq \tau_s$, \ssnote{Fix bound}
     \begin{align}
         | \bar{X}_{\tau} | &< \log (\frac{2}{\delta}) + \log ( \underbrace{ \frac{e^{(1 - \frac{1}{2(D+1)^2}) \log(M_{\bar{V}} M_{\bar{W}})  + \frac{D}{2|| \mathcal{R}^{\dagger}||_2(D+1)^2}}}{1 - e^{-(1 - \frac{1}{2(D+1)^2})(\frac{D}{||\mathcal{R}^{\dagger}||_2} - \log ( M_{\bar{V}} M_{\bar{W}}))}}}_{\mathcal{S}_s}\\
         &\quad + e^{|x_0|} ( e^{|| \mathcal{R} ||_2 D} M_{\bar{V}} M_{\bar{W}} )^{\tau_w} e^{-\frac{1}{2}( \frac{D}{|| \mathcal{R}^{\dagger} ||_2} - \log(M_{\bar{V}} M_{\bar{W}}) )(\tau_s - \tau_w)} e^{-(1 - \frac{1}{2(D+1)^2})( \frac{D}{|| \mathcal{R}^{\dagger} ||_2} - \log(M_{\bar{V}} M_{\bar{W}}) )(\tau - \tau_s)} \\
        & \quad + e^{ \frac{1}{2} ( \frac{D}{|| R^{\dagger} ||_2} + \log (M_{\bar{V}} M_{\bar{W}}) ) } \frac{1 - e^{-\frac{1}{2}(\frac{D}{||\mathcal{R}^{\dagger}||_2} - \log ( M_{\bar{V}} M_{\bar{W}}))(\tau - \tau_w)}}{1 - e^{-\frac{1}{2}(\frac{D}{||\mathcal{R}^{\dagger}||_2} - \log ( M_{\bar{V}} M_{\bar{W}}))}} e^{-(1 - \frac{1}{2(D+1)^2})( \frac{D}{|| \mathcal{R}^{\dagger} ||_2} - \log(M_{\bar{V}} M_{\bar{W}}) )(\tau - \tau_s)}  \\
        & \underbrace{\quad -e^{(1 - \frac{1}{2(D+1)^2}) \log(M_{\bar{V}} M_{\bar{W}})  + \frac{D}{2|| \mathcal{R}^{\dagger}||_2(D+1)^2}} \frac{e^{-(1 - \frac{1}{2(D+1)^2})(\frac{D}{||\mathcal{R}^{\dagger}||_2} - \log ( M_{\bar{V}} M_{\bar{W}}))(\tau - \tau_s)}}{1 - e^{-(1 - \frac{1}{2(D+1)^2})(\frac{D}{||\mathcal{R}^{\dagger}||_2} - \log ( M_{\bar{V}} M_{\bar{W}}))}})}_{\mathcal{T}_s} .
     \end{align}
     Here, $\tau_w = \tilde{O}(\frac{\lambda_{\text{max}}^2(\Sigma_W)}{p^2 \lambda_{\text{min}}(\Gamma_{\text{sb}})g_{\text{sn}}^2})$, and $\tau_s = \tilde{O}(\frac{\lambda_{\text{max}}^2(\Sigma_W)D^6}{p^2 \lambda_{\text{min}}(\Gamma_{\text{sb}})g_{\text{sn}}^2})$. Note that $\tau_w,\tau_s$ are logarithmic factors of $\frac{1}{\delta}$, and thus the dependency on $\delta$ is hidden by $\tilde{O}(\cdot)$.
\end{theorem}

\begin{remark}
    Theorem \ref{theorem:simplified-bound-v2} provides a high probability upper bound on the norm of the sub-sampled states. In particular, bounds are provided over three intervals for $\tau$, which are $[0,\tau_w)$, $[\tau_w,\tau_s)$, and $[\tau_s,\infty)$. We can interpret $[0,\tau_w)$ as the unstable/poorly estimated interval, where the term $\tau_w$ is an upper bound on the time step where the parameter estimate converges into a slightly stabilizing set around the true parameter. Over this region, an upper bound on the states is obtained based on the worst-case behaviour of saturated controls, which can can be seen to grow as a function of $\tau$. 

    We can interpret $[\tau_w,\tau_s)$ as a weakly stable interval, where the system begins to exhibit slightly stable behaviour. The term $\tau_s$ is an upper bound on the time step where the parameter estimate converges into a small set around the true parameter. The weakly stable characteristics can be seen by noting that the bound $\log(\frac{2}{\delta}) + \log (\mathcal{T}_w + \mathcal{T}_s)$ consists of a transient component $\mathcal{T}_w$ which decays to zero, and a steady-state component $\mathcal{S}_w$. Qualitatively speaking, this means that after time step $\tau_w$, our upper bound starts converging towards $\mathcal{S}_w$ as opposed to the unstable interval where it has unbounded growth. `Weakly stable' refers to the fact that here, $\mathcal{S}_w$ is very conservative. \ssnote{Add some more intuition here about SS term}. Note that $\tau_w$ grows at rate $\lambda_{\text{max}}^2(\Sigma_W)$ for large $\lambda_{\text{max}}(\Sigma_W)$, and decays at rate $\frac{1}{p^2 \lambda_{\text{min}}(\Gamma_{\text{sb}})}$ for large $p$ and $\lambda_{\text{min}}(\Gamma_{sb})$. The intuition here is that larger $\lambda_{\text{max}}(\Sigma_W)$ increases the size of the noise in the OLS problem making it more difficulty and resulting in slower parameter convergence to the slightly stabilizing set, and larger $p$, $\lambda_{\text{min}}(\Gamma_{sb})$ increases the size of the signal in the OLS problem, resulting in faster convergence. Moreover, $\tau_w$ decays at rate $\frac{1}{g_{\text{sn}}^2}$ for large noise-signal gap $g_{\text{sn}}$. Intuitively the reason for this is that the set of stabilizing parameter estimates grows for larger $g_{\text{sn}}$ (when $g_{\text{sn}}$ is larger, larger $\epsilon$ can be found which renders $\lambda(\epsilon) < 1$), so a less accurate estimate is required to achieve stability. Qualitatively, this means that $\tau_w$ may be decreased by selecting large additive noise $V_t$ to increase $p$, $\lambda_{\text{min}}(\Gamma_{\text{sb}})$, and large D to increase $g_{\text{sn}}$. Note that $g_{\text{sn}}$ also decreases based on the size of $V_t$, and so the increase in $D$ needs to compensate for this.
    
     We can interpret $[\tau_s,\infty)$ as a strongly stable interval, where the system begins to exhibit strong stability characteristics. The strongly stable characteristics can be seen by noting that the bound $\log(\frac{2}{\delta}) + \log (\mathcal{T}_s + \mathcal{T}_s)$ consists of a transient component $\mathcal{T}_s$ which decays to zero, and a steady-state component $\mathcal{S}_s$. \ssnote{In particular, `strongly stable' is used for this interval since $\mathcal{S}_s$ is tighter than $\mathcal{S}_w$, and moreover, $\mathcal{S}_s$ is monotonically decreasing and converges to $\mathcal{S}_*$ as $D \rightarrow \infty$, where $\mathcal{S}_*$ is the steady state bound in the case where the parameter estimation error is zero.} This captures the idea that for larger $D$, the saturated CE control can use larger controls with larger magnitude to overpower the disturbances in the system, decreasing the spread of the states. The interpretation of the relationship between $\tau_s$ and $\lambda_{\text{max}}(\Sigma_W)$, $p$, $\lambda_{\text{min}}(\Gamma_{\text{sb}})$ is similar to $\tau_w$. However, $\tau_s$ grows at rate $D^6$ for large $D$. The reason for this is because the steady-state value actually scales proportionally with $\epsilon D$ where $\epsilon$ is the estimation error, such that for a fixed $\epsilon$, increasing $D$ will increase the steady-state. This was already observed in $\mathcal{S}_w^{\infty}$, which has unbounded growth as a function of $D$. Thus, in order to capture the idea that $D$ actually decreases the steady state value, $\tau_S$ has been defined as the time that the parameter estimate enters a ball of size $\epsilon$ which decays at rate $1/D^2$ as $D \rightarrow \infty$, such that increasing $D$ will therefore increase $\tau_s$. Although $D$ does show up within $g_{\text{sn}}$, it only appears linearly, so $D^6$ overpowers $g_{\text{sn}}$.
\end{remark}


==> old_estimation_results.tex <==

% \ssnote{READ TO HERE - CAN IGNORE THE REST FOR NOW!!!!}

% \subsection{Finite-Sample Parameter Estimation Error Bounds}

% \begin{definition} \label{def:bmsb}
% (Martingale Small-Ball \cite[Definition 2.1]{simchowitz2018learning}) Given a process $(Z_t)_{t \geq 1}$ taking values in $\mathbb{R}^2$, we say that it satisfies the $(k,\Gamma_{\text{sb}},p)$-block martingale small-ball (BMSB) condition for \ssnote{$k \in \mathbb{N}$}, $\Gamma_{\text{sb}} \succ 0$, and \ssnote{$p > 0$}, if, for any $\zeta \in \mathcal{S}^{1}$ and $j \geq 0$, $\frac{1}{k} \sum_{i=1}^k P (\abs{\langle \zeta, Z_{j+i} \rangle} \geq \sqrt{\zeta^{\top} \Gamma_{\text{sb}} \zeta} \mid \mathcal{F}_j) \geq p$ holds. Here, $(\mathcal{F}_t)_{t \geq 1}$ is any filtration which $(\langle \zeta, Z_{t} \rangle)_{t \geq 1}$ is adapted to.
% \ssnote{Definition needs to be modified to account for higher dimensional data}
% \end{definition}

% \begin{assumption} \label{assump:bmsb}
%     The data sequence $(Z_t)_{t \in \mathbb{N}}$ satisfies the $(k,\Gamma_{\text{sb}},p)$-BMSB condition for some $k > 0$, $\Gamma_{\text{sb}} \succ 0$, and $p > 0$.
% \end{assumption}

% \begin{proposition} \label{prop:param-converge}
%     Consider the sequence of parameter estimates $(\hat{\theta}_{\tau})_{\tau \in \mathbb{N}}$ obtained from \eqref{eqn:dec2022-orthog-ident-parameter-estimate}, and suppose Assumption \ref{assump:bmsb} holds. Then, there exist known functions $M$, $c_1$, $c_2$, $m$ and known constants $\Gamma_{\text{sb}} \succ 0$, $q > 0$, $p > 0$ such that 
%     \begin{equation}
%         P(||\hat{\theta}_{\tau}-\theta_*||_2 > d) \leq \delta_2(t,d,\Gamma_{\text{sb}},q,p)
%     \end{equation}
%     holds for all $d \in (0,m(\Gamma_{\text{sb}},q,p))$ and $\tau \geq M(d,\Gamma_{sb},q,p)$, where  $\delta_2(t,d,\Gamma_{\text{sb}},q,p)=t^{4/3} e^{-c_1(d,\Gamma_{\text{sb}},q,p)t}c_2(d,\Gamma_{\text{sb}},q,p)$. 
%     \ssnote{We may need to modify this result based on the relationship between $\tau$ and $t$ during parameter estimation.}
% \end{proposition}

% \begin{theorem}
% Suppose Assumption \ref{assump:disturbance} holds, $(A,B) \in \mathbb{R}^{n \times n} \times \mathbb{R}^{n \times m}$ satisfy Assumption \ref{assump:reachable}, and Assumption \ref{assump:bmsb} holds. Consider the sequence $(\bar{X}_\tau)_{\tau \in \mathbb{N}_0}$ evolving via the closed-loop system in \eqref{eqn:closed-loop-system}. There exist $d_* > 0$ and $\lambda \in (0,1)$ such that
% \begin{align}
%     | \bar{X}_{\tau} | \leq \ln { (\lambda^{\tau - \tau_0} \mathbb{E}[e^{|\bar{X}_{\tau_0}|}] + \mathbb{E}[e^{|W_0|}]\sum_{i=0}^{\tau - \tau_0 - 1} \lambda^i })
% \end{align}
% holds with at least probability $1 - \delta - \ssnote{S(\tau_0,\tau)}$ for all $\delta \in (0,1)$, $\tau \geq \tau_0 \geq M(d^*,\Gamma_{\text{sb}},q,p)$, where
% \begin{equation}
%     \ssnote{S(\tau_0,\tau) := \sum_{i = \tau_0}^{\tau} i^{4/3} e^{-c_1(d,\Gamma_{sb},q,p)i} c_2(d,\Gamma_{sb},q,p).}
% \end{equation}
% \ssnote{Probably clean this up so that it looks nicer... E.g. not depending on summation symbol.}
% \end{theorem}
